Optimized Generation of Entanglement by Real-Time Ordering of Swapping Operations

Long-distance quantum communication in quantum networks faces significant challenges due to the constraints imposed by the no-cloning theorem. Most existing quantum communication protocols rely on the a priori distribution of entanglement pairs (EPs), a process known to incur considerable latency due to its stochastic nature. In this work, we consider the problem of minimizing the latency of establishing an EP across a pair of nodes in a quantum network. While prior research has primarily focused on minimizing the expected generation latency by selecting {\em static} entanglement routes and/or swapping trees in advance, our approach considers a real-time adaptive strategy -- wherein the order of entanglement-swapping operations (hence, the swapping tree used) is progressively determined at runtime based on the runtime success/failure of the stochastic events. In this context, we present a greedy algorithm that iteratively determines the best route and/or entanglement-swapping operation to perform at each stage based on the current network. We evaluate our schemes on randomly generated networks and observe a reduction in latency of up to 40% from the optimal offline approach.

==> Figures/Hardness.tex <==
\section{NP-Hardness Proof}

\begin{itemize}
    \item Reduction from graph minimum bisection problem. 
\end{itemize}
